Simons Observatory: Characterization of the Large Aperture Telescope Receiver

The Simons Observatory (SO) is a ground-based cosmic microwave background (CMB) survey experiment that currently consists of three 0.42m small-aperture telescopes (SATs) and one 6m large-aperture telescope (LAT), located at an elevation of 5200m in the Atacama Desert in Chile. At the LAT's focal plane, SO will install >62,000 transition-edge sensor detectors across 13 optics tubes (OTs) within the Large Aperture Telescope Receiver (LATR), the largest cryogenic camera ever built to observe the CMB. Here we report on the validation of the LATR in the laboratory and the subsequent dark testing and validation within the LAT. We show that the LATR meets cryogenic, optical, and detector specifications required for high-sensitivity measurements of the CMB. At the time of writing, the LATR is installed in the LAT with six OTs (corresponding to >31,000 detectors), and the LAT mirrors and remaining seven OTs are undergoing development.

==> Latr_paper.tex <==
\section{CR\textsc{edi}T Roles}
We list here the roles and contributions of the authors according to the Contributor Roles Taxonomy (CRediT)\footnote{\url{https://credit.niso.org/}}. \\ 

\noindent\textbf{Tanay Bhandarkar}: Conceptualization (equal), Data curation (equal), Formal analysis (lead), Investigation (lead), Methodology (equal), Resources (equal), Software (equal), Validation (lead), Visualization (equal), Writing - original draft (lead), Writing - review \& editing (lead).\\ 
\textbf{Gabriele Coppi}: Conceptualization (supporting), Investigation (supporting), Methodology (supporting), Resources (supporting), Writing - review \& editing (supporting).\\ 
\textbf{Thomas Satterthwaite}: Conceptualization (supporting), Formal analysis (equal), Investigation (equal), Methodology (supporting), Validation (supporting), Writing - review \& editing (supporting).\\ 
\textbf{Shawn Henderson}: Conceptualization (supporting), Investigation (supporting), Methodology (supporting), Project administration (supporting), Resources (supporting), Software (supporting), Validation (supporting), Writing - review \& editing (supporting).\\ 
\textbf{Federico Nati}: Conceptualization (supporting), Funding acquisition (lead), Investigation (supporting), Methodology (supporting), Resources (supporting), Validation (supporting), Writing - review \& editing (supporting).\\ 
\textbf{Matthew Koc}: Conceptualization (supporting), Investigation (supporting), Methodology (supporting), Resources (supporting), Validation (supporting).\\ 
\textbf{Carlos Sierra}: Conceptualization (supporting), Investigation (supporting), Methodology (supporting), Resources (supporting), Validation (supporting).\\ 
\textbf{Michael Link}: Conceptualization (supporting), Investigation (supporting), Methodology (supporting), Resources (supporting), Validation (supporting), Writing - review \& editing (supporting).\\ 
\textbf{Tammy Lucas}: Conceptualization (supporting), Investigation (supporting), Methodology (supporting), Resources (supporting), Validation (supporting), Writing - review \& editing (supporting).\\ 
\textbf{Michael Vissers}: Conceptualization (supporting), Investigation (supporting), Methodology (supporting), Resources (supporting), Validation (supporting).\\ 
\textbf{Kyuyoung Bae}: Conceptualization (supporting), Investigation (supporting), Methodology (supporting), Resources (supporting), Validation (supporting).\\ 
\textbf{Shannon Duff}: Conceptualization (supporting), Investigation (supporting), Methodology (supporting), Resources (supporting), Validation (supporting), Writing - review \& editing (supporting).\\ 
\textbf{Jenna Moore}: Conceptualization (supporting), Investigation (supporting), Methodology (supporting), Resources (supporting), Validation (supporting), Writing - review \& editing (supporting).\\ 
\textbf{Tran Tsan}: Conceptualization (supporting), Methodology (supporting), Software (supporting), Validation (supporting), Writing - review \& editing (supporting).\\ 
\textbf{Liam Walters}: Conceptualization (supporting), Validation (supporting), Writing - review \& editing (supporting).\\ 
\textbf{Jason Austermann}: Conceptualization (supporting), Resources (supporting), Validation (supporting), Writing - review \& editing (supporting).\\ 
\textbf{Eve Vavagiakis}: Conceptualization (supporting), Resources (supporting), Validation (supporting), Writing - review \& editing (supporting).\\ 
\textbf{Zeeshan Ahmed}: Conceptualization (supporting), Formal analysis (supporting), Funding acquisition (supporting), Investigation (supporting), Methodology (supporting), Project administration (supporting), Resources (supporting), Supervision (supporting), Writing - review \& editing (supporting).\\ 
\textbf{Brian Koopman}: Conceptualization (supporting), Software (supporting), Writing - review \& editing (supporting).\\ 
\textbf{Nicholas Galitzki}: Conceptualization (supporting), Methodology (supporting), Writing - review \& editing (supporting).\\ 
\textbf{Daniel Dutcher}: Conceptualization (supporting), Investigation (supporting), Methodology (supporting), Resources (supporting), Software (supporting), Validation (supporting), Writing - review \& editing (supporting).\\ 
\textbf{Mark Devlin}: Conceptualization (supporting), Funding acquisition (lead), Investigation (supporting), Methodology (equal), Project administration (lead), Resources (lead), Supervision (lead), Writing - review \& editing (supporting).\\ 
\textbf{Robert Thornton}: Conceptualization (supporting), Investigation (supporting), Methodology (supporting), Project administration (supporting), Resources (supporting), Validation (supporting), Writing - review \& editing (supporting).\\ 
\textbf{Simon Dicker}: Conceptualization (supporting), Investigation (supporting), Methodology (supporting), Resources (supporting), Validation (supporting), Writing - review \& editing (supporting).\\ 
\textbf{John Orlowski-Scherer}: Conceptualization (supporting), Formal analysis (supporting), Investigation (supporting), Methodology (supporting), Validation (supporting), Writing - review \& editing (supporting).\\ 
\textbf{Yuhan Wang}: Conceptualization (supporting), Data curation (equal), Formal analysis (supporting), Investigation (supporting), Methodology (supporting), Resources (supporting), Software (supporting), Validation (supporting), Writing - review \& editing (supporting).\\ 
\textbf{Anna Kofman}: Conceptualization (supporting), Formal analysis (supporting), Investigation (supporting), Methodology (supporting), Resources (equal), Software (supporting), Validation (supporting), Visualization (supporting), Writing - review \& editing (supporting).\\ 
\textbf{Saianeesh Haridas}: Conceptualization (supporting), Data curation (equal), Formal analysis (equal), Investigation (supporting), Methodology (equal), Resources (equal), Software (equal), Validation (supporting), Visualization (supporting), Writing - original draft (supporting), Writing - review \& editing (supporting).\\ 
\textbf{Jon Gudmundsson}: Conceptualization (supporting), Resources (supporting), Validation (supporting), Visualization (supporting), Writing - review \& editing (supporting).\\ 
\textbf{Karen Perez Sarmiento}: Conceptualization (supporting), Data curation (supporting), Investigation (supporting), Methodology (supporting), Software (supporting), Validation (supporting), Writing - original draft (supporting).\\ 
\textbf{Mario Zannoni}: Conceptualization (supporting), Funding acquisition (supporting), Investigation (supporting), Methodology (supporting), Resources (supporting), Validation (supporting), Writing - review \& editing (supporting).\\ 
\textbf{Michele Limon}: Conceptualization (supporting), Investigation (supporting), Methodology (supporting), Project administration (supporting), Supervision (supporting), Validation (supporting), Visualization (supporting).\\ 
\textbf{Suzanne Staggs}: Conceptualization (supporting), Funding acquisition (supporting), Methodology (supporting), Project administration (supporting), Resources (supporting), Supervision (supporting), Validation (supporting).\\ 
\textbf{Michael Niemack}: Conceptualization (supporting), Funding acquisition (supporting), Methodology (supporting), Project administration (supporting), Resources (supporting), Supervision (supporting), Validation (supporting), Writing - review \& editing (supporting).\\
\\

